Whispering Experts: Neural Interventions for Toxicity Mitigation in Language Models

An important issue with Large Language Models (LLMs) is their undesired ability to generate toxic language. In this work, we show that the neurons responsible for toxicity can be determined by their power to discriminate toxic sentences, and that toxic language can be mitigated by reducing their activation levels proportionally to this power. We propose AUROC adaptation (AurA), an intervention that can be applied to any pre-trained LLM to mitigate toxicity. As the intervention is proportional to the ability of each neuron to discriminate toxic content, it is free of any model-dependent hyperparameters. We show that AurA can achieve up to $2.2 \times$ reduction in toxicity with only a $0.72$ perplexity increase. We also show that AurA is effective with models of different scale (from 1.5B to 40B parameters), and its effectiveness in mitigating toxic language, while preserving common-sense zero-shot abilities, holds across all scales. AurA can be combined with pre-prompting strategies, boosting its average mitigation potential from $1.28\times$ to $2.35\times$. Moreover, AurA can counteract adversarial pre-prompts that maliciously elicit toxic content, making it an effective method for deploying safer and less toxic models.

==> bkp/method_pieter.tex <==

\subsection{Emergence of Toxic Experts Neurons}
\label{sec:emergence}

The literature on expert units focuses on small language models, \emph{i.e.},  GPT-2, and concise concepts (\eg WordNet senses). 
% This setting is far from our goal, that is to reduce toxicity in recent large language models.
As a preliminary set of experiments, we probe if analogous experts appear in language models for more complex concepts, specifically we check for toxicity. 
To understand the presence of experts in larger language models beyond GPT-2, we test for toxic experts over a wide range of parameters.
We find experts for the MPT-7B, MPT-30B~\citep{MosaicML2023Introducing} , Falcon~\citep{falcon40b}, Mosaic-7B
and a wide range of OPT~\citep{zhang2022opt} models using both the HateCheck and Jigsaw 2018 benchmarks as probing datasets.
% Due to licensing restrictions, we can not compare to either version LlaMa, but given the performance of MPT and Falcon on various benchmarks, we argue that these are good replacements.

\paragraph{Concept removal is more effective on larger models.}
We measure the Average Precision (AP) on each benchmark (Jigsaw and HateCheck) when removing the top 5k expert units identified by \method.
Higher AP means lower toxicity or hate speech.
% In Figure~\ref{fig:hate-experts}, we show the trend of removing a fixed number of experts as we grow  models on their level of toxicity. 
In \autoref{fig:hate-experts}, we show the average AP of the top 5k expert units as we increase the model size, for both benchmarks.
We observe that as LLM size increases, the toxicity expert units are better at detecting toxic content and increasingly specialize, and  hence, removing the top experts has a more positive impact on larger models. \xs{bold assertion. We must point to Falcon-40B results or remove or say its a conjecture.}
Note that we purposely only look at a small number of experts -- 5k -- that represents only 5\% of the smallest model with 350M parameters. 
The increasing AP trend with model size indicates that the part of the network responsible for concepts like hate speech becomes more specialized and identifiable as a model grows in size.
This observation complements that of~\citet{zhang-2022-language} that toxicity increases with model size, leading to the following conclusion: \emph{as larger models become more toxic, the internal mechanisms responsible for toxicity are easier to identify}.
A possible hypothesis is that larger models have more ``room'' to specialize neurons, rather than being bottle-necked to employ them for multiple tasks or concepts, and larger models increasingly act as an implicit mixtures of experts.

%\aj{merge figure 1 and 2 to summarize trend on both dataset. No need to put all the subcategories in main paper.}\pieter{ok, I'll make a combined chart and we can put those in the appendices.}

\subsection{Reducing Toxicity with Expert Neurons}

% \begin{table}[t]
% \centering
% \caption{\textbf{Toxicity reduction.} Comparison between \method~and several baselines across architectures. We evaluate the generation of hurtful continuations (HONEST) and toxic continuations (RTP).}
% \label{tab:comparision}
% \begin{tabular}{@{}llllll@{}}
% \toprule
%                                      &           & \multicolumn{2}{c}{\textbf{RealToxicityPrompts}  ($\downarrow$)}\\ \cmidrule(l){3-4}
% \textbf{Method}     & Perplexity                 & \textbf{HONEST} ($\downarrow$)                            & Toxic prob.             & Toxic cont. (\%)\\ 
% \midrule
% \textbf{GPT2-XL}                     &                            &                          &                  \\
% No intervention     & 39.1                 & 0.2166                     & 0.054                    & 0.29\%           \\%\\ 39.1
% DExperts           & 99.2 \ua{153\%}                 & \textbf{0.0451} \da{79\%}                      & 0.005 \da{91\%}                    &       0.026   \da{91\%}      \\ % 99.192
% CTRL            & 176.9 \ua{352\%}                    & 0.2230 \ua{3\%}                    & \textbf{0.047} \da{13\%}                & \textbf{0.24\%} \da{17\%}          \\ %176.9
% \method      &  43.8 \ua{12\%}                     & 0.1971    \da{9.0\%}          & \textbf{0.047} \da{13\%}                & \textbf{0.24\%}  \da{17\%}         \\ %PPL: 43.88762234202957
% \midrule
% \textbf{MPT-7B}                      &                            &                          &                  \\
% No intervention    & 41.7                  & 0.2243                     & 0.041                    &        0.20\%          \\ %41.7
% \selfcond        &    41.6  \da{0.2\%}                   & \textbf{0.2202} \da{1.8\%} & 0.035 \da{15\%}          &       ??           \\ %41.6
% \method        &     42.8  \ua{2.6\%}                & \textbf{0.2146} \da{4.3\%} & \textbf{0.020} \da{51\%} &     0.097\%  \da{52\%}           \\ %42.8
% \midrule
% \textbf{Falcon-7B}                   &                            &                          &                  \\
% No intervention     & 43.3                 & 0.2381                     & 0.055                    & 0.33\%           \\ %43.3
% %Prompts                              & 0.2801                     & 0.069 \ua{25\%}          & 0.39\% \ua{18\%} \\ 23.7
% Prompts            & 37.5 \da{13\%}                 & \textbf{0.0834} \da{65\%}                     & 0.016 \da{71\%}          & 0.10\% \da{70\%} \\ % PPL: 37.457
% \method      & 44.0  \ua{1.6\%}                      & 0.2326    \da{2.3\%}                 & {0.023} \da{58\%} & 0.12\% \da{64\%} \\
% %\method~+ prompts    & 0.2597                     & 0.034 \da{38\%}          & 0.16\% \da{48\%}  \\ \bottomrule
% \method~+ prompts & 37.5 \da{13\%}  & 0.0837  \da{65\%}                   & \textbf{0.011} \da{80\%}          & 0.06\% \da{82\%}  \\ \bottomrule %37.524
% \end{tabular}
% \end{table}


% TABLE WITH E[neg] BELOW

% \begin{table}[t]
% % \centering
% \caption{\textbf{Toxicity reduction.} Comparison between \method~and several baselines across architectures. We evaluate the generation of hurtful continuations (HONEST) and toxic continuations (RTP).}
% \label{tab:comparision}
% \begin{tabular}{@{}lllllll@{}}
% \toprule
% & &       &    & \multicolumn{2}{c}{\textbf{RealToxicityPrompts}}\\ \cmidrule(l){5-6}
% Model & Method     & \textbf{PPL} ($\downarrow$)                & \textbf{HONEST} ($\downarrow$)                            & Prob. ($\downarrow$)             & Toxic cont. ($\downarrow$)\\ 
% \midrule

% % \textbf{GPT2-XL}                     &                            &                          &                  \\
% \multirow{4}{*}{GPT2-XL} & No intervention     & 38.6                 & 0.221                     & 0.066                 & 0.374\%           \\%\\ 39.1
% & DExperts           & 39.7 \ua{2.8\%}                 & {0.204} \da{7.7\%}                      & 0.0302 \da{54\%}                    &       0.173\%  \da{53\%}      \\ % 99.192
% & CTRL            & 176.9 \ua{358\%}                    & 0.223 \ua{0.8\%}                    & {0.047} \da{29\%}                & {0.240\%} \da{35\%}          \\ %176.9
% & \method      &  39.2 \ua{1.6\%}                     &  0.203    \da{8.1\%}          & {0.036} \da{45\%}                & {0.206\%}  \da{45\%}         \\ %k=5169
%  \midrule


% % % \textbf{GPT2-XL}                     &                            &                          &                  \\
% % \multirow{4}{*}{GPT2-XL} & No intervention     & 38.6                 & 0.221                     & 0.066                 & 0.374\%           \\%\\ 39.1
% % & DExperts           & 53.1 \ua{38\%}                 & {0.134} \da{39\%}                      & 0.017 \da{74\%}                    &       0.090\%  \da{76\%}      \\ % 99.192
% % & CTRL            & 176.9 \ua{358\%}                    & 0.223 \ua{0.8\%}                    & {0.047} \da{29\%}                & {0.240\%} \da{35\%}          \\ %176.9
% % &\best \method      & \best 39.6 \ua{2.6\%}                     & \best 0.215    \da{3.0\%}          &\best {0.049} \da{26\%}                &\best {0.258\%}  \da{31\%}         \\ %k=5169
% %  \midrule

 
% \multirow{3}{*}{MPT-7B} & No intervention    & 41.7                  & 0.224                     & 0.041                    &        0.202\%          \\ %41.7
% & \selfcond        &    42.1  \ua{1.0\%}                   & {0.229} \ua{2.1\%} & 0.030 \da{27\%}          &       0.145\%  \da{27\%}         \\ %41.6
% & \best\method        &     \best 43.7  \ua{4.8\%}                &\best 0.192 \da{14\%} & \best {0.009} \da{78\%} &     \best 0.043\%  \da{78\%}           \\ %11014
%  \midrule
% \multirow{3}{*}{MPT-30B} & No intervention    & 43.6                  & 0.196                     & 0.057                    &        0.326\%          \\ %41.7
% & \selfcond        &    43.6 \na{\hspace{1ex}= \hspace{1ex}}                  & {0.191} \da{2.6\%} & 0.056 \da{1.8\%}          &       0.319\%  \da{2.1\%}         \\ %41.6
% & \best\method        &     \best 48.1  \ua{10\%}                &\best 0.185 \da{5.6\%} & \best {0.009} \da{84\%} &     \best 0.046\%  \da{86\%}           \\ %44668

% \midrule
% \multirow{3}{*}{Falcon-7B} & No intervention     & 43.4                 & 0.243                   & 0.062                    & 0.338\%           \\ %43.3
% & \selfcond      & 43.2  \da{0.4\%}                      & 0.247    \ua{2.1\%}                 & 0.049\da{21\%} & 0.273\% \da{19\%} \\
% & \best \method      & \best 44.5  \ua{2.5\%}                      & \best 0.218    \da{10\%}                 & \best 0.014\da{77\%} & \best0.076\% \da{77\%} \\ %11014
% \midrule
% \multirow{3}{*}{Falcon-40B} & No intervention     & 44.5                 & 0.235                   & 0.058                    & 0.324\%           \\ %43.3
% & \selfcond      & 44.8  \ua{0.7\%}                      & 0.211    \da{10\%}                 & {0.049} \da{16\%} & 0.269\% \da{17\%} \\
% & \best\method      & \best 45.6  \ua{2.4\%}                      & \best0.169    \da{28\%}                 & \best 0.011\da{81\%} & \best 0.070\% \da{78\%} \\ %22610

% \midrule
% \multirow{5}{*}{Falcon-7B-i} & No intervention     & 44.5                 & 0.235                   & 0.065                    & 0.324\%           \\ %43.3
% & \selfcond      & 44.6  \da{0.2\%}                      & 0.265    \ua{6\%}                 & {0.062} \da{4.6\%} & 0.347\% \da{2.5\%} \\
% & \method      & 49.1  \ua{5.1\%}                      & 0.224    \da{10\%}                 & {0.026} \da{60\%} & 0.130\% \da{63\%} \\ %11014
% & Prompt           & 37.6 \da{19\%}                 & {0.078} \da{69\%}                     & 0.014 \da{78\%}          & 0.100\% \da{72\%} \\ % 
% %\method~+ prompts    & 0.2597                     & 0.034 \da{38\%}          & 0.16\% \da{48\%}  \\ \bottomrule
% %\rowcolor{SeaGreen3!30!}
% & \best\method~+ prompt & \best38.0 \da{19\%}  & \best0.090  \da{64\%}                   & \best{0.005} \da{92\%}          & \best0.042\% \da{88\%}  \\ \bottomrule %11014
% \end{tabular}
% \end{table}


% TABLE WITH ZERO BELOW


\begin{table}[t]
% \centering
\caption{\textbf{Toxicity reduction.} Comparison between \method~and several baselines across architectures. We evaluate the generation of hurtful continuations (HONEST) and toxic continuations (RTP).}
\label{tab:comparision}
\begin{tabular}{@{}lllllll@{}}
\toprule
& &       &    & \multicolumn{2}{c}{\textbf{RealToxicityPrompts}}\\ \cmidrule(l){5-6}
Model & Method     & \textbf{PPL_{WIK}} ($\downarrow$)                & \textbf{HONEST} ($\downarrow$)                            & Prob. ($\downarrow$)             & Toxic cont. ($\downarrow$)\\ 

% & CTRL            & 176.9 \ua{608\%}                    & 0.223 \ua{0.9\%}                    & {0.047} \da{21\%}                & {0.240\%} \da{30\%}          \\ %176.9


% GPT2-XL ours 48000
% GPT2-XL selfcond 8000
% DExperts DExperts 20
% Falcon-7B ours 20500
% Falcon-7B selfcond 2000
% Falcon-40B ours 32000
% Falcon-40B selfcond 0
% MPT-7B ours 15000
% MPT-7B selfcond 1000
% MPT-30B ours 32000
% MPT-30B selfcond 3000
% Mistral-7B ours 11500
% Mistral-7B selfcond 12000
% Falcon-7B-i ours 20500
% Falcon-7B-i ours-i 26000
% Falcon-7B-i selfcond 3000
% Falcon-7B-i selfcond-i 2000
% \midrule
% \multirow{4}{*}{GPT2-XL} & No intervention  & 29.1 & 0.221 & 0.060 & 0.346\% \\
%  & DExperts  & 30.6 \ua{5.1\%} & 0.204 \da{9.0\%} & 0.030 \da{45.9\%} & 0.173\% \da{46.1\%} \\
%  & \selfcond  & 28.8 \da{0.8\%} & 0.228 \ua{3.0\%} & 0.050 \da{16.4\%} & 0.274\% \da{20.8\%} \\
%  & \method  & 31.1 \ua{7.1\%} & 0.113 \da{48.9\%} & 0.004 \da{93.3\%} & 0.018\% \da{94.9\%} \\

% \midrule
% \multirow{3}{*}{Falcon-7B} & No intervention  & 8.8 & 0.247 & 0.051 & 0.305\% \\
%  & \selfcond  & 8.8 \na{=} & 0.222 \da{10.3\%} & 0.040 \da{21.2\%} & 0.224\% \da{26.5\%} \\
%  & \method  & 9.6 \ua{8.2\%} & 0.161 \da{34.9\%} & 0.006 \da{88.6\%} & 0.034\% \da{89.0\%} \\

% \midrule
% \multirow{3}{*}{Falcon-40B} & No intervention  & 7.3 & 0.232 & 0.059 & 0.333\% \\
%  & \selfcond  & 7.3 \na{=} & 0.231 \na{=} & 0.051 \da{12.9\%} & 0.296\% \da{11.1\%} \\
%  & \method  & 7.9 \ua{9.1\%} & 0.188 \da{19.1\%} & 0.015 \da{74.1\%} & 0.109\% \da{67.3\%} \\

% \midrule
% \multirow{3}{*}{MPT-7B} & No intervention  & 5.9 & 0.236 & 0.038 & 0.198\% \\
%  & \selfcond  & 5.9 \na{=} & 0.224 \da{5.1\%} & 0.026 \da{30.3\%} & 0.134\% \da{32.7\%} \\
%  & \method  & 6.3 \ua{6.6\%} & 0.174 \da{26.3\%} & 0.007 \da{81.4\%} & 0.040\% \da{79.8\%} \\

% \midrule
% \multirow{3}{*}{MPT-30B} & No intervention  & 5.6 & 0.202 & 0.059 & 0.332\% \\
%  & \selfcond  & 5.6 \na{=} & 0.187 \da{7.6\%} & 0.046 \da{21.4\%} & 0.260\% \da{21.7\%} \\
%  & \method  & 5.9 \ua{4.9\%} & 0.160 \da{21.0\%} & 0.012 \da{79.6\%} & 0.067\% \da{79.8\%} \\

% \midrule
% \multirow{3}{*}{Mistral-7B} & No intervention  & 8.4 & 0.193 & 0.047 & 0.280\% \\
%  & \selfcond  & 8.8 \ua{4.7\%} & 0.145 \da{25.1\%} & 0.005 \da{90.2\%} & 0.026\% \da{90.6\%} \\
%  & \method  & 8.4 \na{=} & 0.167 \da{13.7\%} & 0.011 \da{76.2\%} & 0.066\% \da{76.6\%} \\

% \midrule
% \multirow{5}{*}{Falcon-7B-i} & No intervention  & 11.9 & 0.241 & 0.058 & 0.337\% \\
%  & \selfcond  & 11.9 \na{=} & 0.207 \da{14.0\%} & 0.037 \da{37.1\%} & 0.178\% \da{47.0\%} \\
%  & \method  & 13.0 \ua{9.4\%} & 0.151 \da{37.2\%} & 0.008 \da{86.9\%} & 0.041\% \da{87.9\%} \\
% [1pt]\cdashline{2-6}[.6pt/2pt] \\ [-9pt]
%  & Prompt  & 19.5 & 0.077 & 0.015 & 0.102\% \\
%  & Prompt + \method  & 19.4 \na{=} & 0.087 \ua{12.9\%} & 0.002 \da{88.0\%} & 0.015\% \da{85.0\%} \\

\midrule
\multirow{4}{*}{GPT2-XL} & \textit{No interv.}  & \textit{29.07} & \textit{0.221} & \textit{0.060} & \textit{0.346\% }\\
 & DExperts  & 30.55 \ua{1.49} & 0.204 \da{$1.1\times$} & 0.030 \da{$1.8\times$} & 0.173\% \da{$1.9\times$} \\
 & \selfcond  & 28.84 \da{0.23} & 0.228 \da{$1.0\times$} & 0.050 \da{$1.2\times$} & 0.274\% \da{$1.3\times$} \\
 & \method  & 28.22 \da{0.85} & 0.122 \da{$1.8\times$} & 0.005 \da{$11.5\times$} & 0.024\% \da{$14.4\times$} \\

\midrule
\multirow{3}{*}{Falcon-7B} & \textit{No interv.}  & \textit{8.84} & \textit{0.247} & \textit{0.051} & \textit{0.305\% }\\
 & \selfcond  & 8.82 \da{0.02} & 0.222 \da{$1.1\times$} & 0.040 \da{$1.3\times$} & 0.224\% \da{$1.4\times$} \\
 & \method  & 10.31 \ua{1.48} & 0.138 \da{$1.8\times$} & 0.003 \da{$19.6\times$} & 0.015\% \da{$20.1\times$} \\

\midrule
\multirow{3}{*}{Falcon-40B} & \textit{No interv.}  & \textit{7.26} & \textit{0.232} & \textit{0.059} & \textit{0.333\% }\\
 & \selfcond  & 7.26 \na{=} & 0.231 \da{$1.0\times$} & 0.051 \da{$1.1\times$} & 0.296\% \da{$1.1\times$} \\
 & \method  & 8.32 \ua{1.06} & 0.162 \da{$1.4\times$} & 0.006 \da{$10.5\times$} & 0.039\% \da{$8.5\times$} \\

\midrule
\multirow{3}{*}{MPT-7B} & \textit{No interv.}  & \textit{5.89} & \textit{0.236} & \textit{0.038} & \textit{0.198\% }\\
 & \selfcond  & 5.92 \ua{0.03} & 0.224 \da{$1.1\times$} & 0.026 \da{$1.4\times$} & 0.134\% \da{$1.5\times$} \\
 & \method  & 6.57 \ua{0.68} & 0.172 \da{$1.4\times$} & 0.005 \da{$8.2\times$} & 0.022\% \da{$8.9\times$} \\

\midrule
\multirow{3}{*}{MPT-30B} & \textit{No interv.}  & \textit{5.61} & \textit{0.202} & \textit{0.059} & \textit{0.332\% }\\
 & \selfcond  & 5.62 \ua{0.01} & 0.187 \da{$1.1\times$} & 0.046 \da{$1.3\times$} & 0.260\% \da{$1.3\times$} \\
 & \method  & 6.31 \ua{0.70} & 0.144 \da{$1.4\times$} & 0.009 \da{$6.8\times$} & 0.046\% \da{$7.3\times$} \\

\midrule
\multirow{3}{*}{Mistral-7B} & \textit{No interv.}  & \textit{8.40} & \textit{0.193} & \textit{0.047} & \textit{0.280\% }\\
 & \selfcond  & 8.79 \ua{0.39} & 0.145 \da{$1.3\times$} & 0.005 \da{$10.2\times$} & 0.026\% \da{$10.6\times$} \\
 & \method  & 8.37 \da{0.02} & 0.167 \da{$1.2\times$} & 0.011 \da{$4.2\times$} & 0.066\% \da{$4.3\times$} \\

\midrule
\multirow{5}{*}{Falcon-7B-i} & \textit{No interv.}  & \textit{11.88} & \textit{0.241} & \textit{0.058} & \textit{0.337\% }\\
 & \selfcond  & 11.89 \ua{0.01} & 0.207 \da{$1.2\times$} & 0.037 \da{$1.6\times$} & 0.178\% \da{$1.9\times$} \\
 & \method  & 13.38 \ua{1.50} & 0.142 \da{$1.7\times$} & 0.005 \da{$12.7\times$} & 0.020\% \da{$16.8\times$} \\
[1pt]\cdashline{2-6}[.6pt/2pt] \\ [-9pt]
 & Prompt  & 19.50 \ua{7.62} & 0.077 \da{$3.1\times$} & 0.015 \da{$3.9\times$} & 0.102\% \da{$3.3\times$} \\
 & Prompt + Ours  & 19.42 \ua{7.54} & 0.087 \da{$2.8\times$} & 0.002 \da{$32.3\times$} & 0.015\% \da{$22.2\times$} \\

\bottomrule
\end{tabular}
\end{table}

We evaluate how toxicity decreases with our intervention on toxicity experts. 
We consider two sets of benchmarks. %(1) the standard benchmark to compare with existing methods, and (2) a set of evaluations with recent large language models.
For the first set, we follow the evaluation pipeline of~\citet{keskar2019ctrl} and use a GPT-2 XL with 1.5B parameters.
For the second set, we focus on two 7B parameters models, MPT-7B and Falcon-7B, and we compare with prompting as a baseline.
The motivation is to measure the difference of impact of our approach on a base and instruct finetuned models.
In Table~\ref{tab:comparision}, we report the results on Honest and RealToxicityPrompts~(RTP), as well as, in terms of perplexity (PPL) to control if the impact of intervention on the generation.

\paragraph{Comparison with existing work on GPT-2.} We compare \method~with CTRL (1.5B parameters) and a similar-sized model (GPT2-XL, 1.5B parameters) with no intervention (Table~\ref{tab:comparision} top row).
Our approach slightly improves over CTRL on HONEST and is on par on RTP.
Both methods improve over the original model.
This experiment validates that our approach is competitive with existing work, and we can further test it with larger models.

\paragraph{Comparision on base and instruction finetuned 7B LLMs.}
On these models, we observe that our approach reduces toxicity with a factor of 2x to 5x on both benchmarks. 
It is worth noting that the prompt already has a positive effect with a reduction of toxicity of 71\% on RTP. %finetuned model, Falcon-7B, is slightly more toxic that the base MPT-7B model on both benchmarks.
%We report two baselines, that are the original set of experts, \textbf{E-Set} and prompting the model with a text that explicitly encourage non-toxic generation.
We compare \method~to \textbf{\selfcond}, and our anti-toxic instruction prompt on MTP-7B and Falcon-7B.
Overall, we observe that \method~has the greater impact on toxicity reduction on both benchmarks, espcially on RTP.
We are comparable with \textbf{\selfcond} on HONEST, which is expected since this dataset is composed of simple generated toxic and non-toxic sentences.
On the other hand, when we work on the more challenging prompts contained in the RTP benchmark, we observe that our modification to the original \textbf{\selfcond} approach has a greater impact.
%We observe that our approach does not compare favorably with a prompt tailored for Falcon-7B and these dataset by ourselves.
While our anti-toxic prompt outperforms \method~on RTP, combing the two methods greatly improves the toxicity of Falcon-7B
However, combining both approaches slightly improve over this prompt.
Note that using prompts that were tailored for another model does not work as well, and we even observed degraded performance in preliminary experiments.
Nonetheless, the conclusion of this experiment is that, when prompting is available and can be tailored to a specific model, prompt is superior.


\subsubsection{Impact of interventions on standard benchmarks}
Although our method is effective at reducing toxicity, we %validate if this is achieved by reducing the generative capacity of the model (e.g. outputting nonsensical tokens) or if targeting only selected neurons can maintain this generative capacity.
%We find that there is a slight increase in perplexity (+1.8\%)  when intervening on 11k units, see
%\autoref{tab:downstream}.
%Given the large number of intervened units, this is a small increase over the original \selfcond version, where the perplexity would increase to 60.9 for the same number of experts (see \autoref{ss:ablation} for the discussion on the number of experts).
%In this set of experiments, w
also assess the impact of modifying the internal mechanisms of a LLM on different benchmarks that are not related to toxicity.
Our goal is to validate if modifying a neuron that is marked as toxic, does not create undesired effect on domain where we would not want to intervene. 
To do so, we consider perplexity on RTP generations and 5 different benchmarks that are available in the Eleuther benchmark harness\footnote{\url{https://github.com/EleutherAI/lm-evaluation-harness}}.

In \autoref{tab:downstream}, we show that \method~has a relatively low impact on the model perplexity across benchmark tasks.
In some cases, we even observe a small improvement, that suggests there is a level of uncertainty associated with these benchmarks and small changes are not significant.
As a point of comparison, \textbf{\selfcond} has a negative impact on performance, showing that their intervention may be too coarse and affect other areas beyond toxicity.


\section{Ablation study}

In this section we explore how our intervention affects the model's utility, 


%First, we investigate further how our intervention affects the model's utility.
%The results in \autoref{tab:comparision} show that our method does not degrade perplexity, however  our intervention might still hurt zero-shot performance.
%To this end, we test how our method performs on
%We test this by evaluating perplexity again, but on a dataset not related to toxicity, and with 
%two zero-shot common-sense reasoning tasks  (\autoref{ss:utility}).

First,
we analyze the effect of varying the number of experts that we intervene on, as well as the impact of our soft forcing hyperparameter $\alpha$.
(\autoref{ss:ablation})

Second, we test our hypothesis that mitigating toxicity in larger language models would perform better, since the experts we target are better as well.
To test this, we compare the performance of toxicity mitigation on both Falcon-7B and Falcon-40B.
We expect to see a lower toxicity for the same perplexity (\autoref{ss:bigger-models})

Finally,
we perform an ablation study on our method to understand the effects of the choices we made. 
More precisely we consider the original approach of setting expert activations to zero, using either the toxic or non-toxic examples for experts (\autoref{ss:negatives}).


%\begin{table}[]
%\centering
%\caption{Results of our method and the original experts for toxicity mitigation. We evaluate the generation of hurtful continuations (HONEST) and using RealToxicity prompts, we evaluate the perplexity (PPL) and toxic continuations (RTP).}
%\label{tab:toxicity-mitigation}
%\resizebox{0.7\columnwidth}{!}{%
%\begin{tabular}{@{}llll@{}}
%\toprule
%\textbf{Method}       & \textbf{HONEST} & \textbf{PPL} & \textbf{RTP} \\ \midrule
%\textbf{MPT-7B}      & && \\
%No intervention & 0.2243          & 41.7       & 0.041       \\
%25 \selfcond        & \textbf{0.2202} \da{1.8\%} & \textbf{41.6} \da{0.2\%} & 0.035 \da{15\%}    \\
%11k \selfcond       & 0.3025 \ua{34.9\%} & 60.9 \ua{46.0\%} & 0.420 \ua{1024.4\%}    \\
%25 \method & 0.2287\ua{2.0\%}  & 41.7 \na{\hspace{1ex}=\hspace{1ex} } &  0.036 \da{12\%}    \\
%11k \method & \textbf{0.2202}\da{1.8\%} & 42.5 \ua{1.8\%} & \textbf{0.020} \da{51\%}   \\ \midrule
%
%\textbf{MPT-30B}      & x               & x            & x            \\
%11k{\color{red}??} \selfcond              & x (+ y\%)       & x (+ y\%)    & x (+ y\%)    \\
%11k{\color{red}??} \method & x (+ y\%)       & x (+ y\%)    & x (+ y\%)    \\ \bottomrule
%\end{tabular}
%}
%\end{table}


%\begin{table}[]
%\centering
%\caption{UTILITY TABLE Evaluation of the utility of our models and the original experts. Aside from the perplexity (PPL), we also evaluate two zero-shot common-sense reasoning tasks (PIQA and SIQA).}
%\label{tab:downstream}
%\resizebox{\linewidth}{!}{%
%\begin{tabular}{@{}lllllll@{}}
%\toprule
%\textbf{Method}                           & \textbf{PPL} & \textbf{PIQA} & \textbf{SIQA} &\textbf{TRIVIAQA} & \textbf{TRUTHFULQA} & \textbf{HELLASWAG} \\ %\midrule
%\textbf{Method}                           & {$\downarrow$} & {$\uparrow$} & {$\uparrow$} &{$\uparrow$} & {$\uparrow$} & {$\uparrow$} \\ \midrule
%\textbf{MPT-7B}                           & &&\\
%No intervention & x            & 79.2$\pm$ 0.9             & 42.0$\pm$ 1.1  & 0.275 $\pm$ 0.0033 &  0.2044$\pm$ 0.0141, mc2=0.334$\pm$0.0130 & 0.57179$\pm$  0.0049      \\
%11k \selfcond                                 & x     & 74.5 $\pm$ 1.0 \dab{6.0\%}    & 39.8$\pm$ 1.1 \dab{5.2\%}   & . &  . & .      \\
%\method & x (+ y\%)    & 78.7$\pm$ 1.0 \dab{0.6\%}     & 41.3$\pm$ 1.1 \dab{1.7\%} & 0.288 $\pm$ 0.003 & 0.219 $\pm$ 0.014, mc2=0.344$\pm$0.013 & 0.56$\pm$0.005   \\ \midrule
%%\textbf{MPT-30B}                          & x            & x             & x       & . &  . & .         \\
%%\selfcond                                 & x (+ y\%)    & x (+ y\%)     & x (+ y\%)   & . &  . & .     \\
%%\method & x (+ y\%)    & x (+ y\%)     & x (+ y\%)     \\ \bottomrule
%\end{tabular}%
%}
%\end{table}


% \usepackage{tabularray}
% \begin{table}
% \centering
% \caption{\textbf{Impact of removing toxic neurons on standard benchmarks.} Evaluation of the utility of our models and the original experts. Aside from the perplexity (PPL), we also evaluate two zero-shot common-sense reasoning tasks (PIQA and SIQA).}
% \label{tab:downstream}
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{@{}lllllll@{}}
% \toprule
%  &             & \textbf{PIQA} ($\uparrow$)             & \textbf{SIQA} ($\uparrow$)            & \sc{\textbf{TriviaQA}} ($\uparrow$)  & \sc{\textbf{TruthfulQA}} ($\uparrow$)                     & \sc{\textbf{Hellaswag}} ($\uparrow$)  \\
% \textbf{Method} & \textbf{PPL} ($\downarrow$)             & Accuracy                & Accuracy                & Exact match (\%) & Mult. Choice                               &Accuracy          \\ \midrule
% \textbf{MPT-7B} &                          &                            &                           &                    &                                          &                     \\
% No interv. & 41.7                     & \textbf{79.2}\small{$\pm$ 0.9}              & 42.0\small{$\pm$ 1.1}             & 27.5\small{ $\pm$ 0.3} & 0.20\small{ $\pm$ 0.01} & 57.1\small{ $\pm$ 0.5} \\
% \selfcond       & \textbf{41.6} \da{0.2\%}     & 74.5\small{$\pm$ 1.0} \dab{6.0\%} & 39.8\small{$\pm$ 1.1} \dab{5.2\%} & 27.3\small{ $\pm$ 0.3} \dab{0.8\%} & 0.20\small{ $\pm$ 0.01} \na{\hspace{1ex}=\hspace{1ex} }  & \textbf{57.7}\small{ $\pm$ 0.5} \uag{1\%}               \\
% \method         & 42.8 \ua{2.6\%}          & 78.7\small{$\pm$ 1.0} \dab{0.6\%}  & 41.3\small{$\pm$ 1.1} \dab{1.7\%} & \textbf{28.8}\small{ $\pm$ 0.3} \uag{4.7\%}  & \textbf{0.22}\small{ $\pm$ 0.01} \uag{10\%}    & 56.1\small{ $\pm$ 0.5} \dab{1.8\%}  \\ \midrule

% \textbf{Falcon-7B} &                          &                            &                           &                    &                                          &                     \\
% No interv. & 43.3                    & 79.5\small{$\pm$ 0.9}              & 42.2\small{$\pm$ 1.1}             & 38.3\small{ $\pm$ 0.4} & 0.22\small{ $\pm$ 0.01} & \textbf{57.8}\small{ $\pm$ 0.5} \\
% \selfcond       &      & 78.9\small{$\pm$ 1.0} \dab{0.7\%} & 41.6\small{$\pm$ 1.1} \dab{1.4\%} & \textbf{40.7}\small{$\pm$ 0.4} \uag{6.3\%} & \textbf{0.23}\small{$\pm$ 0.01} \uag{4.5\%}  & 55.6\small{ $\pm$ 0.5} \dab{3.8\%}               \\
% \method         & 44.0 \ua{\%}          & \textbf{79.7}\small{$\pm$ 1.0} \uag{0.2\%}  & \textbf{42.7}\small{$\pm$ 1.1} \uag{1.2\%} & 35.1\small{ $\pm$ 0.4} \dab{8.3\%}  & \textbf{0.23}\small{ $\pm$ 0.01} \uag{4.5\%}    & 56.7\small{ $\pm$ 0.5} \dab{1.9\%} 
%    \\ \bottomrule   
% \end{tabular}
% }
% \end{table}







% \begin{table}
% \centering
% \caption{\textbf{Impact of removing toxic neurons on standard benchmarks.} Evaluation of the utility of our models and the original experts. Aside from the perplexity (PPL), we also evaluate two zero-shot common-sense reasoning tasks (PIQA and SIQA).}
% \label{tab:downstream}
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{@{}lllllll@{}}
% \toprule
%  &             & \textbf{PIQA} ($\uparrow$)             & \textbf{SIQA} ($\uparrow$)            & \sc{\textbf{TriviaQA}} ($\uparrow$)  & \sc{\textbf{TruthfulQA}} ($\uparrow$)                     & \sc{\textbf{Hellaswag}} ($\uparrow$)  \\
% \textbf{Method} & \textbf{PPL} ($\downarrow$)             & Accuracy                & Accuracy                & Exact match (\%) & Mult. Choice                               &Accuracy          \\ \midrule

% \textbf{GPT2-XL} &                          &                            &                           &                    &                                          &                     \\
% No interv. & \textit{38.6}                     & 
% \textit{70.9} $\pm$ \textit{1.1} & \textit{38.9} $\pm$ \textit{1.1} & \textit{6.0} $\pm$ \textit{0.2} & \textit{22.0} $\pm$ \textit{1.5} & \textit{40.0} $\pm$ \textit{0.5} \\
% % \selfcond       & \textbf{41.6} \da{0.2\%}     & 
% % 54.6 $\pm$ 1.2\dab{22.9\%} & 34.0 $\pm$ 1.1\dab{12.6\%} & 0.0 $\pm$ 0.0\dab{99.6\%} & 21.7 $\pm$ 1.4\dab{1.7\%} & 25.8 $\pm$ 0.4\dab{35.6\%} \\
% \method         & 39.6 \ua{2.6\%} & 
% 70.7 $\pm$ 1.1\dab{0.3\%} & 38.9 $\pm$ 1.1\uag{0.1\%} & 5.1 $\pm$ 0.2\dab{15.2\%} & 22.6 $\pm$ 1.5\uag{2.8\%} & 39.4 $\pm$ 0.5\dab{1.6\%} \\
% \midrule


% \textbf{Falcon-7B} &                          &                            &                           &                    &                                          &                     \\
% No interv. & \textit{43.4 }                    & 
% \textit{79.5} $\pm$ \textit{0.9} & \textit{42.2} $\pm$ \textit{1.1} & \textit{38.2} $\pm$ \textit{0.4} & \textit{22.3} $\pm$ \textit{1.5} & \textit{57.8} $\pm$ \textit{0.5} \\
% % \selfcond       & 43.2 \da{0.4\%}     & 
% % 79.5 \pm 0.9\na{\hspace{1ex}=\hspace{1ex} } & 41.9 \pm 1.1\dab{0.7\%} & 37.4 \pm 0.4\dab{2.1\%} & 22.4 \pm 1.5\uag{0.4\%} & 57.6 \pm 0.5\dab{0.3\%} \\
% \method         & 44.5 \ua{2.5\%} & 
% 79.8 \pm 0.9\uag{0.4\%} & 42.4 \pm 1.1\uag{0.5\%} & 30.8 \pm 0.3\dab{19.4\%} & 24.1 \pm 1.5\uag{8.1\%} & 57.1 \pm 0.5\dab{1.2\%} \\
% \midrule

% \textbf{Falcon-40B} &                          &                            &                           &                    &                                          &                     \\
% No interv. & \textit{44.5}                     & 
% \textit{82.3} $\pm$ \textit{0.9} & \textit{45.0} $\pm$ \textit{1.1} & \textit{52.7} $\pm$ \textit{0.4} & \textit{27.5} $\pm$ \textit{1.6} & \textit{64.0} $\pm$ \textit{0.5} \\
% % \selfcond       & 44.8 \ua{0.7\%}     & 
% % 81.4 \pm 0.9\dab{1.0\%} & 43.1 \pm 1.1\dab{4.2\%} & 49.2 \pm 0.4\dab{6.7\%} & 25.9 \pm 1.5\dab{5.8\%} & 62.1 \pm 0.5\dab{3.0\%} \\
% \method         & 45.6 \ua{2.4\%} & 
% 81.2 \pm 0.9\dab{1.3\%} & 45.2 \pm 1.1\uag{0.5\%} & 48.3 \pm 0.4\dab{8.5\%} & 29.0 \pm 1.6\uag{5.3\%} & 63.3 \pm 0.5\dab{1.1\%} \\
% \midrule

% \textbf{MPT-7B} &                          &                            &                           &                    &                                          &                     \\
% No interv. & \textit{41.7}                     & 
% \textit{79.4} $\pm$ \textit{0.9} & \textit{41.9} $\pm$ \textit{1.1} & \textit{27.5} $\pm$ \textit{0.3} & \textit{20.4} $\pm$ \textit{1.4} & \textit{57.2} $\pm$ \textit{0.5} \\
% % \selfcond       & \textbf{42.1} \da{1.0\%}     & 
% % 79.2 \pm 0.9\dab{0.3\%} & 41.8 \pm 1.1\dab{0.2\%} & 27.3 \pm 0.3\dab{0.4\%} & 21.1 \pm 1.4\uag{3.0\%} & 56.6 \pm 0.5\dab{1.0\%} \\
% \method         & 43.7 \ua{4.8\%} & 
% 78.8 \pm 1.0\dab{0.8\%} & 42.0 \pm 1.1\uag{0.1\%} & 24.8 \pm 0.3\dab{9.6\%} & 22.8 \pm 1.5\uag{11.4\%} & 56.3 \pm 0.5\dab{1.6\%} \\
% \midrule

% \textbf{MPT-30B} &                          &                            &                           &                    &                                          &                     \\
% No interv. & \textit{43.6}                     & 
% \textit{80.5} $\pm$ \textit{0.9} & \textit{43.5} $\pm$ \textit{1.1} & \textit{52.8} $\pm$ \textit{0.4} & \textit{25.8} $\pm$ \textit{1.5} & \textit{60.9} $\pm$ \textit{0.5} \\
% % \selfcond       & 43.6 \na{\hspace{1ex}=\hspace{1ex} }     & 
% % 80.3 \pm 0.9\dab{0.3\%} & 43.5 \pm 1.1\na{\hspace{1ex}=\hspace{1ex} } & 52.7 \pm 0.4\dab{0.3\%} & 26.7 \pm 1.5\uag{3.3\%} & 60.3 \pm 0.5\dab{0.9\%} \\
% \method         & 48.1 \ua{10\%} & 
% 80.4 \pm 0.9\dab{0.1\%} & 43.6 \pm 1.1\uag{0.1\%} & 49.2 \pm 0.4\dab{6.9\%} & 26.6 \pm 1.5\uag{2.8\%} & 59.6 \pm 0.5\dab{2.1\%} \\
% \bottomrule   
% \end{tabular}
% }
% \end{table}




\begin{table}
\centering
\caption{\textbf{Impact of removing toxic neurons on perplexity of toxic and non-toxic datasets.} Evaluations of the perplexity of different models with and without interventions. We evaluate on neutral corpora (WIK, MIS and UNC) and on different toxic datasets. We observe that the perplexity remains low and unchanged for neutral corpora and increases for the toxic ones.}
\label{tab:downstream}
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}llll;{.6pt/2pt}lllllll@{}}
\toprule

\textbf{Method} & PPL_{WIK}  & PPL_{MIS}  & PPL_{UNC}  & PPL_{TX}  & PPL_{STX}  & PPL_{IDH}  & PPL_{THR}  & PPL_{INS}  & PPL_{OBS} \\

\midrule
\textbf{GPT2-XL}  & & & & & & & & & \\
No interv.  & \textit{29.1}  & \textit{50.8}  & \textit{34.1}  & \textit{195.7}  & \textit{189.1}  & \textit{158.5}  & \textit{110.4}  & \textit{204.6}  & \textit{207.3} \\
\method  & \textbf{31.1} \na{$1.1\times$}  & \textbf{55.5} \na{$1.1\times$}  & 44.0 \na{$1.3\times$}  & 744.3 \na{$3.8\times$}  & 1126.2 \na{$6.0\times$}  & 687.1 \na{$4.3\times$}  & 475.5 \na{$4.3\times$}  & 891.6 \na{$4.4\times$}  & 935.6 \na{$4.5\times$} \\
\midrule
\textbf{Falcon-7B}  & & & & & & & & & \\
No interv.  & \textit{8.8}  & \textit{35.1}  & \textit{18.5}  & \textit{172.3}  & \textit{123.9}  & \textit{469.8}  & \textit{80.2}  & \textit{211.0}  & \textit{207.5} \\
\method  & \textbf{9.6} \na{$1.1\times$}  & \textbf{34.5} \na{$1.0\times$}  & \textbf{19.9} \na{$1.1\times$}  & 350.8 \na{$2.0\times$}  & 340.3 \na{$2.7\times$}  & 826.1 \na{$1.8\times$}  & 176.6 \na{$2.2\times$}  & 447.3 \na{$2.1\times$}  & 438.5 \na{$2.1\times$} \\
\midrule
\textbf{Falcon-40B}  & & & & & & & & & \\
No interv.  & \textit{7.3}  & \textit{25.8}  & \textit{15.8}  & \textit{137.8}  & \textit{98.2}  & \textit{198.4}  & \textit{83.4}  & \textit{153.2}  & \textit{158.7} \\
\method  & \textbf{7.9} \na{$1.1\times$}  & \textbf{28.3} \na{$1.1\times$}  & \textbf{17.0} \na{$1.1\times$}  & 120588.7 \na{$875.1\times$}  & 554.7 \na{$5.7\times$}  & 1044.6 \na{$5.3\times$}  & 272.6 \na{$3.3\times$}  & 236718.2 \na{$1545.0\times$}  & 217896.5 \na{$1373.3\times$} \\
\midrule
\textbf{MPT-7B}  & & & & & & & & & \\
No interv.  & \textit{5.9}  & \textit{22.3}  & \textit{17.3}  & \textit{193.1}  & \textit{223.9}  & \textit{136.6}  & \textit{90.1}  & \textit{233.2}  & \textit{243.8} \\
\method  & \textbf{6.3} \na{$1.1\times$}  & \textbf{23.6} \na{$1.1\times$}  & \textbf{19.0} \na{$1.1\times$}  & 409.9 \na{$2.1\times$}  & 541.8 \na{$2.4\times$}  & 325.9 \na{$2.4\times$}  & 171.0 \na{$1.9\times$}  & 552.7 \na{$2.4\times$}  & 571.5 \na{$2.3\times$} \\
\midrule
\textbf{MPT-30B}  & & & & & & & & & \\
No interv.  & \textit{5.6}  & \textit{22.1}  & \textit{18.2}  & \textit{163.1}  & \textit{129.0}  & \textit{129.0}  & \textit{106.6}  & \textit{172.5}  & \textit{185.9} \\
\method  & \textbf{5.9} \na{$1.0\times$}  & \textbf{22.9} \na{$1.0\times$}  & \textbf{19.3} \na{$1.1\times$}  & 376.3 \na{$2.3\times$}  & 563.5 \na{$4.4\times$}  & 352.8 \na{$2.7\times$}  & 195.0 \na{$1.8\times$}  & 467.2 \na{$2.7\times$}  & 495.5 \na{$2.7\times$} \\
\midrule
\textbf{Mistral-7B}  & & & & & & & & & \\
No interv.  & \textit{8.4}  & \textit{36.1}  & \textit{36.1}  & \textit{484.5}  & \textit{581.9}  & \textit{500.1}  & \textit{352.0}  & \textit{520.6}  & \textit{560.0} \\
\method  & \textbf{8.4} \na{$1.0\times$}  & \textbf{35.7} \na{$1.0\times$}  & \textbf{35.7} \na{$1.0\times$}  & 685.6 \na{$1.4\times$}  & 992.5 \na{$1.7\times$}  & 764.8 \na{$1.5\times$}  & 486.0 \na{$1.4\times$}  & 785.7 \na{$1.5\times$}  & 835.3 \na{$1.5\times$} \\



\bottomrule   
\end{tabular}
}
\end{table}



\begin{table}
\centering
\caption{\textbf{Impact of removing toxic neurons on standard benchmarks.} Evaluation of the utility of our models and the original experts. Aside from the perplexity (PPL), we also evaluate two zero-shot common-sense reasoning tasks (PIQA and SIQA).}
\label{tab:downstream}
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}llllll@{}}
\toprule
             & \textbf{PIQA} ($\uparrow$)             & \textbf{SIQA} ($\uparrow$)            & \sc{\textbf{TriviaQA}} ($\uparrow$)  & \sc{\textbf{TruthfulQA}} ($\uparrow$)                     & \sc{\textbf{Hellaswag}} ($\uparrow$)  \\
\textbf{Method} ($\downarrow$)             & Accuracy                & Accuracy                & Exact match (\%) & Mult. Choice                               &Accuracy          \\ 

\midrule
\textbf{GPT2-XL} & & & & & \\
No interv. & \textit{70.9} $\pm$ \textit{1.1} & \textit{38.9} $\pm$ \textit{1.1} & \textit{6.0} $\pm$ \textit{0.2} & \textit{38.5} $\pm$ \textit{1.4} & \textit{40.0} $\pm$ \textit{0.5} \\
Ours & 65.6 $\pm$ 1.1\dab{7.5\%} & 37.5 $\pm$ 1.1\dab{3.7\%} & 1.7 $\pm$ 0.1\dab{71.5\%} & 42.6 $\pm$ 1.5\uag{10.5\%} & 35.4 $\pm$ 0.5\dab{11.7\%} \\


\midrule
\textbf{Falcon-7B} & & & & & \\
No interv. & \textit{79.5} $\pm$ \textit{0.9} & \textit{42.2} $\pm$ \textit{1.1} & \textit{38.2} $\pm$ \textit{0.4} & \textit{34.3} $\pm$ \textit{1.3} & \textit{57.8} $\pm$ \textit{0.5} \\
Ours & 78.2 $\pm$ 1.0\dab{1.6\%} & 42.8 $\pm$ 1.1\uag{1.6\%} & 24.6 $\pm$ 0.3\dab{35.8\%} & 39.8 $\pm$ 1.4\uag{16.3\%} & 55.8 $\pm$ 0.5\dab{3.4\%} \\


\midrule
\textbf{Falcon-40B} & & & & & \\
No interv. & \textit{82.3} $\pm$ \textit{0.9} & \textit{45.0} $\pm$ \textit{1.1} & \textit{52.7} $\pm$ \textit{0.4} & \textit{41.6} $\pm$ \textit{1.4} & \textit{64.0} $\pm$ \textit{0.5} \\
Ours & 81.6 $\pm$ 0.9\dab{0.9\%} & 45.4 $\pm$ 1.1\uag{0.9\%} & 48.0 $\pm$ 0.4\dab{9.1\%} & 46.2 $\pm$ 1.4\uag{11.0\%} & 63.7 $\pm$ 0.5\dab{0.5\%} \\


\midrule
\textbf{MPT-7B} & & & & & \\
No interv. & \textit{79.4} $\pm$ \textit{0.9} & \textit{41.9} $\pm$ \textit{1.1} & \textit{27.5} $\pm$ \textit{0.3} & \textit{33.4} $\pm$ \textit{1.3} & \textit{57.2} $\pm$ \textit{0.5} \\
Ours & 78.4 $\pm$ 1.0\dab{1.3\%} & 42.3 $\pm$ 1.1\uag{1.0\%} & 16.7 $\pm$ 0.3\dab{39.1\%} & 37.3 $\pm$ 1.4\uag{11.7\%} & 56.0 $\pm$ 0.5\dab{2.1\%} \\


\midrule
\textbf{MPT-30B} & & & & & \\
No interv. & \textit{80.5} $\pm$ \textit{0.9} & \textit{43.5} $\pm$ \textit{1.1} & \textit{52.8} $\pm$ \textit{0.4} & \textit{38.4} $\pm$ \textit{1.4} & \textit{60.9} $\pm$ \textit{0.5} \\
Ours & 80.4 $\pm$ 0.9\dab{0.1\%} & 44.4 $\pm$ 1.1\uag{2.0\%} & 44.6 $\pm$ 0.4\dab{15.6\%} & 38.8 $\pm$ 1.4\uag{1.1\%} & 59.8 $\pm$ 0.5\dab{1.8\%} \\


\midrule
\textbf{Mistral-7B} & & & & & \\
No interv. & \textit{80.5} $\pm$ \textit{0.9} & \textit{42.7} $\pm$ \textit{1.1} & \textit{59.3} $\pm$ \textit{0.4} & \textit{42.6} $\pm$ \textit{1.4} & \textit{61.2} $\pm$ \textit{0.5} \\
Ours & 81.1 $\pm$ 0.9\uag{0.7\%} & 42.5 $\pm$ 1.1\dab{0.5\%} & 59.5 $\pm$ 0.4\uag{0.4\%} & 43.1 $\pm$ 1.4\uag{1.0\%} & 61.2 $\pm$ 0.5\dab{0.0\%} \\

\bottomrule   
\end{tabular}
}
\end{table}


\subsection{Effect of hyperparameters: number of experts and $\alpha$}\label{ss:ablation}
We vary the number of activated expert units, where we compare the trade-off between toxicity and perplexity---which has been shown in \autoref{tab:downstream} to be a good proxy for downstream task performance. We focus our analysis on MPT-7B, although we did observe similar behaviour with Falcon-7B.


\autoref{fig:pareto-mpt} shows the effect of varying the number of experts when targeting toxicity experts (green line) and other sets of experts (see \autoref{ss:negatives}). Up until 11k experts, the toxiciy decreases while maintaining the same perplexity as without intervention. However, after this point, the model starts generating text with higher toxicity and higher perplexity. These are often repetitions of tokens that can be considered toxic, but without any coherence.



\autoref{fig:alpha}: hyperparam alpha (details in \autoref{ss:alpha})


\begin{figure}[tb]
     \centering
     \begin{subfigure}[t]{0.49\linewidth}
         \centering
         \centering
        \includegraphics[width=\linewidth]{figures/Falcon-40B_alpha_sweep_ppl (normalized).pdf}
        \caption{}
        % \caption{Impact of $\alpha$ in \autoref{eq:do-ours}. Note that $\alpha\approx 0.5$ shows an empirically good trade-off between toxicity mitigation and perplexity.}
        \label{fig:pareto-mpt-models}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/falcon-7b-random-experts.pdf}
        \vspace{-2mm}
        \caption{}
         % \caption{Pareto front of toxicity mitigation with respect to perplexity, as the numbers of expert neurons $k$ is increased for Falcon-7B. Choosing the top-k experts is a sensible choice, as compared to 5 evaluations with randomly chosen experts.}
        \label{fig:pareto-mpt}
     \end{subfigure}
% \caption{Pareto frontiers of different types of experts (\autoref{fig:pareto-mpt}) and different methods to suppress the experts (\autoref{fig:pareto-mpt-models}). All evaluations are done using MPT-7B while varying the number of experts between 0 (no intervention) and 50k.}\label{fig:hyperparams}
\caption{(a) Impact of $\alpha$ in \autoref{eq:do-ours}. Note that $\alpha\approx 0.5$ shows an empirically good trade-off between toxicity mitigation and perplexity. (b) Pareto front of toxicity mitigation with respect to perplexity, as the numbers of expert neurons $k$ is increased for Falcon-7B. Choosing the top-k experts is a sensible choice, as compared to 5 evaluations with randomly chosen experts.}\label{fig:hyperparams}
\end{figure}


\subsection{Model size}\label{ss:bigger-models}
In this section, 


\subsection{Intervening on toxic neurons or negative counterparts}\label{ss:negatives}

See \autoref{fig:pareto-mpt}


\section{Related Work}

We give a brief overview of the relevant literature on measuring and reducing toxicity and biases in language models, as well as, on changing the behavior of a network with internal interventions.

\paragraph{Measuring toxicity and social biases.} 
Generating text with large language models can lead to toxic and biased content~\citep{nadeem2020stereoset, delobelle-etal-2022-measuring}, and most recent advances in language modeling come with an investigation of these issues~\citep{radford2018improving,radford2019language,zhang2022opt,touvron2023llama}.
These investigations rely on standardized benchmarks that were either designed for sentence encoders~\citep{may2019measuring,zhao2019gender,basta2019evaluating,kurita2019measuring} or generation with a language model~\citep{nangia2020crows, nadeem2020stereoset,sheng2019woman, gehman2020realtoxicityprompts,welbl2021challenges,ju2022learning}.
However, defining and thus measuring these issues is complex~\citep{jacobs2021measurement} and studies have highlighted the danger of taking results from these benchmarks  at face value~\citep{blodgett2021stereotyping}, or worse, leveraging them as a form of guarantee of safety~\cite{delobelle-etal-2022-measuring}.
In this work, we follow the recommendations of~\citet{delobelle-etal-2022-measuring} in our selection of benchmarks and how to report results.

\paragraph{Reducing toxicity and social biases.}
Some works reduce toxic generation by modifying the pre-training data~\citep{keskar2019ctrl, korbak2023pretraining}, but most of the literature focuses on controlling the generation of pre-trained networks~\cite{xu2020recipes}.
In particular, the dominant approach is to finetune the network into a safer version, using either supervised examples or reinforcement learning with human feedback~\citep{adolphs2022cringe, bai2022training,zeldes2020technical,ziegler2019fine,chung2022scaling,ouyang2022training}.
Finetuning produces a single language model -- e.g., a chatbot like ChatGPT or Claude -- and hence, can only fit a single set of safety guidelines.
It is thus not adapted to the case where we have different guidelines for different communities. 
Alternatives closer to our work, add a safety component on top of a fixed network by either filtering its output~\citep{dathathri2019plug, xu2020recipes, krause2020gedi, yang2021fudge} or pre-prompting its generation~\cite{li2021prefix,liu2022p}.
These approaches are more flexible, i.e., they can fit any community standards without modifying the network.
Our work follows the same principles and complements existing work by modifying internal mechanisms instead of external quantities.
This type of internal interventions is a promising alternative to pre-prompting for few-shot learning ~\citep{liu2022few}.
 
% \texttt{=====LONG VERSION=====}

%  methods can be placed in three main categories~\citep{zhang2022survey}: 1)~\textit{Fine-tuning} methods train LMs on additional data either to add  additional conditioning weights~\citep{zeldes2020technical}, prompt or prefix tuning~\citep{li2021prefix}, using reinforcement learning to align the weights with user preferences~\citep{ziegler2019fine}, or to directly optimize the model on a dataset crafted for the task of following instructions~\citep{chung2022scaling,ouyang2022training}. 2)~\textit{Re-training} methods like CTRL~\citep{keskar2019ctrl} showed it is also possible to train a model from scratch to take control codes along with the input. Instead of retraining the whole architecture, it is also possible to train a series of conditioning modules~\citep{chan2020cocon}. 3)~\textit{Post-processing} methods consider a frozen LM and focus on guiding text generation towards a desired outcome. For example, PPLM~\citep{dathathri2019plug} leverages the gradient of a small classifier trained on a conditioning variable to guide the sampling process. Instead of gradients, GeDi~\citep{krause2020gedi} leverages a class-conditional generator turned into a class discriminator to bias LM's generation towards the correct class while \citet{yang2021fudge} directly train a discriminator in FUDGE. Different from PPLM, GeDi, or FUDGE, which are applied on top of any pre-trained model, the EBM proposed by \citet{deng2020residual} are trained along with a frozen LM, thus interfering less with the original outputs.
 
% \texttt{===============}

% While the methods described above are promising avenues for CTG, 1) and 2) incur in computational overhead associated to the backward pass in large LMs, while 3) can decrease the text fluency \citep{welbl2021challenges,krause2020gedi,suau2022self}. In this work, we investigate an emerging family of methods based on the use of expert units to condition LMs~\citep{suau2022self,dai-etal-2022-knowledge} as they have potential to generate fluent text without requiring any training.

\paragraph{Expert units and pruning.} 
The seminal work of~\citet{radford2017learning} shows the existence of \textit{sentiment units} in language models. 
These units can be manipulated to induce a positive or negative sentiment in the output. 
\citet{suau2022self} generalize these \textit{expert units} to arbitrary concepts by measuring the response of units to positive and negative examples.
This approach modifies the behavior of the network while perturbing only a fractions of its units, leading to a smaller impact on the perplexity than post-processing approaches, such as FUDGE~\citep{yang2021fudge} and PPLM-BoW~\citep{dathathri2019plug}. 
This study is a proof-of-concept, and, tackling complex concepts such as toxicity or biases, requires several improvements on the original approach.
Our internal manipulations are also related to pruning where the goal is to extract a smaller network without impacting the overall performance~\cite{joulin2016fasttext,zhu2017prune,voita2019analyzing}.
Pruning can achieve high compression rate but, sometimes, at the cost of dropping some important modes in the distribution~\citep{hooker2019compressed}, inducing undesired algorithmic biases~\cite{hooker2020characterising}.
However, this shortcoming is, in our case, a benefit: our goal is precisely to modify the behavior of the network rather than preserving it.
We hope that our findings will encourage more exploration of pruning as a potential solution to toxicity reduction.


\section{Limitations and Future Work}
The primary limitation of \method~is that its performance decreases with the number of LLM parameters. This means that the ideal method to mitigate toxicity is dependent on the size model and \method~does not provide a ``one size fits all'' solution. However, in general, larger LLM's have better performance and are currently the most commonly used and, therefore, important to mitigate toxicity in. Additionally, while \method's computational requirements are low relative to fine tuning a LLM, computation is needed to identify expert units and determine their average precision. Finally, activating the positive concepts (i.e. the toxicity) works up to a certain point, after that the generations become less high-quality (higher PPL) and actually quite toxic. The negative ones don't have this issue, but at the cost of higher perplexity. Finding a better way of combining both would be great.

As future work, using the experts to permanently alter the weights of the model itself (such as through a pruning strategy) would allow for models to be released with low toxicity built in. Additionally, future work should better understand the connections between expert units to avoid new experts appearing as the initially identified experts are suppressed.

% - works less well for smaller models (e.g. GPT2)

% - altough we don't need to train any additional classifiers or retrain the model, we do need to find the exper units.

% - On larger models, this still requires some computions to perform inference and calculate AP for every unit to find experts.

% - Although we used a small number of positive and negative samples ($\leq$250), there might be benefits to using larger sets as well and consider more than AP.

% - activating the positive concepts (i.e. the toxicity) works up to a certain point, after that the generations become less high-quality (higher PPL) and actually quite toxic. The negative ones don't have this issue, but at the cost of higher perplexity. Finding a better way of combining both would be great.

- definition of toxicity: \citet{waseem-etal-2017-understanding}


Future work could focus on:

- altering the weights of the model itself to be able to release a model with reduced toxicity or other properties. A pruning strategy?

- Iterating over the found experts, as suppressing some experts might cause other experts to emerge.


\section{Conclusion}
\Pieter{This section will be the standard conclusion about our work}

\section*{Ethics Statement}
- big models get less toxic without retraining, I call that a win.

- still not fully understood, so activating too many experts can cause harmful content to apear more often instead of less.

\section*{Reproducibility Statement}
Our source code is available at {\tt url removed for double blind review}. To aid reproducibility, we made additional efforts to compare and use a publicly released model for RealToxicityPrompts, instead of the Perspective API that could change without notice. {\color{red}We also provide an illustratory PyTorch implementation in the appendices of \method.}

%\section*{Ethical Considerations}

% \section*{Acknowledgements}
% We thank:
% - Orevaoghene Ahia: suggesting RealToxicityPrompts


==> mean_variance.tex <==


\section{Interventions and variance}
\xs{Just writing things down, disconnected from paper at this point.}

Let $\rz$ be the RV \textit{output of an expert neuron}. The dampening intervention $\hat{\rz} = (1-\alpha) \rz$ reduces both the mean and the variance of $\rz$ by $(1-\alpha)$ and $(1-\alpha)^2$ respectively. This coupling might not be optimal.
We can explore a disentangled intervention on both mean and variance.

Intervention on the mean only, fixing $\E[\hat{\rz}] = \mu$:
\begin{equation}
    \hat{\rz} = \rz - \E[\rz] + \mu.
\end{equation}

Intervention on the variance only, fixing $\Var[\hat{\rz}] = \beta$:
\begin{equation}
    \hat{\rz} = (1 - \alpha)\big(\rz - \E[\rz]\big) + \E[\rz] = (1 - \alpha)\rz + \alpha\E[\rz] \quad \text{with} \quad \alpha = 1-\sqrt{\frac{\beta}{\Var[\rz]}}
\end{equation}

Intervention on both mean and variance, fixing $\E[\hat{\rz}] = \mu$ and $\Var[\hat{\rz}] = \beta$:
\begin{equation}
    \hat{\rz} = (1 - \alpha)\big(\rz - \E[\rz]\big) + \mu  \quad \text{with} \quad \alpha = 1-\sqrt{\frac{\beta}{\Var[\rz]}}
\end{equation}
